Teamwork Makes TEE Work: Open and Resilient Remote Attestation on Decentralized Trust

Remote Attestation (RA) enables the integrity and authenticity of applications in Trusted Execution Environment (TEE) to be verified. Existing TEE RA designs employ a centralized trust model where they rely on a single provisioned secret key and a centralized verifier to establish trust for remote parties. This model is however brittle and can be untrusted under advanced attacks nowadays. Besides, most designs only have fixed procedures once deployed, making them hard to adapt to different emerging situations and provide resilient functionalities. Therefore, we propose JANUS, an open and resilient TEE RA scheme. To decentralize trust, we, on one hand, introduce Physically Unclonable Function (PUF) as an intrinsic root of trust (RoT) in TEE to directly provide physical trusted measurements. On the other hand, we design novel decentralized verification functions on smart contract with result audits and RA session snapshot. Furthermore, we design an automated switch mechanism that allows JANUS to remain resilient and offer flexible RA services under various situations. We provide a UC-based security proof and demonstrate the scalability and generality of JANUS by implementing an complete prototype.

==> backup.tex <==



% without extra overhauls.

% TEE
% it can naturally solve this problem. Therefore,  


% structure unclonability

% The transition from single-party to multi-party endorsement of a measurement can occur in two ways: multi-party measuring or multi-party signing.


% Due to the response pseudo- and , PUF provides , rendering it a unique and independent trust anchor. 

% Thus, PUF can realize measuring and "signing" simultaneously. 


% Integrating PUF into measuring procedure enhances trust basis and only brings small overhead. Such double-layer measurement also coincides with Intel TDX \cite{IntelTrustDomain}.

% Moreover, as a standalone chip, PUF cannot be altered by the TEE manufacturer (even the PUF manufacturer) so 


For the first limitation, However, their decentralization does not stem from the underlying RoT and is still built on the exclusive trust on TEE manufacturers. SCRAPS \cite employ blockchain technique only focus on defending against untrusted verifiers. 

They do not go further to address the trust centralization issue, essentially the root cause of untrust verification. 



This model is the most common of RA and widely adopted in plenty of real-world TEE RA designs [x][x][x]. However, note that must trust TEE manufacturer to true of signature and measurements. users and verifiers must trust the xx first to xiangxin RA. 



% it is still the TEE in TPM or cryptographic means are not feasible here. Software too expensive. New techniques are required for Need new Insight to providing xxx to set extra RoT in TEE RA.

% In traditional TEE RA schemes, such as SGX \cite{costan2016intel}, the TEE manufacturer generates and endorses the measurement and the cryptographic proof, while also molding and using the RoT. Verifiers have to solely trust the manufacturer to validate the measurements. This centralized RoT construction undermines the trustworthiness of attestation and may cause the single point of untrust risk.

% The former would use additional hardware components to measure the status and interoperate with installed TEE. For the latter, we can use cryptographic techniques such as multi-signatures and secret sharing. 



%  is  It hosts  by a user XX. XXX would request a verification service (verifier) to ask $\att$ to return XX's memory measurement with cryptographic proof. Then xx can assure its data integraity by the output results of verifier. 



% Also, verifiers solely execute verification behavior, it output results are hard to be validate by . For users, centralized trust on either attester device or verifier's output. and regulated procedure limits a scenario.  Therefore, traditional TEE RA solutions face two severe limitations in practice. 
% 

% Through RA, various stakeholders, such as cloud service providers, data owners, and developers, can use TEEs assuredly in hostile environments. 




\ie, a verifier or a third-party service. Real-world RA solutions, such as Intel, Azure \cite{azurera}, and AWS \cite{awsra}, claim to maintain the objectivity of the verification service \cite{intelamber} but all contradictively adopt a centralized design. 

The verification service provider could collude with other parties in RA, \eg, the manufacturer, resulting in users never learning the genuine status of their applications: a compromised one may be claimed to be trusted or vice versa. Consequently, traditional TEE RA schemes are built upon a closed and centralized chain of trust, which undermines their trustworthiness and violates the very purpose of remote attestation.



Also, the concentrated trust in manufacturers could indulge them in installing backdoors and trojans to invade uses' applications. 

secrets devices and compromising the beginning of entire supply chain.



Intel SGX, ARM TrustZone and AMD SEV are all by to leak the isolated key. Therefore, the single centralized RoT has been proven to be insecure for . 



advanced side-channel attacks or , The compromised RoT directly leads to the security breach of all xxx. This





Therefore, the TEE RA would to provide trusted results for users.


The Root of Trust (RoT) in TEE is provisioned solely by the manufacturer,

The single and centralized RoT for TEEs in practice is 

with the TEE manufacturer as the only trusted party and endorsing both the measurement and signature. 

The concentrated trust in manufacturers could indulge them in installing backdoors and trojans on devices and compromising the beginning of entire supply chain. Any secret code and data would be extractable for them. Avoiding a single closed RoT is urgently needed to design open TEE functions \cite{KohlbrennerOpenTrusted}. Practical efforts have been made to alleviate this pain point through open-source silicon \cite{opentitan} and specifications \cite{Caliptra}.




% RA assess the trust levels of devices based on their hardware configurations, which can be the reference to audit their historic attestation results.
% We realize a smart contract for turnout to allow participants to freely determine the attestation approach under different conditions or customized requirements.
% We use an Dell EMC server and an NXP LPC55S69 board with Hyperledger Sawtooth \cite{olsonSawtoothIntroduction2018}. And we instantiate a (8-8) IPUF \cite{nguyen2019interpose} in Xilinx FPGA. 

% It offers enhanced security features and consistent performance for large-scale networks. 

% his turnout mechanism enables \janus\ to provide continuous RA services both on-chain and off-chain, making it adaptable to various scenarios.


RATF

IETF


RA systems rely on a trusted component— a trust anchor—for measuring and signing response reports, or quotes, from V. Increasingly, constrained devices are equipped with CPU security extensions from which trust anchors can be built with hardware-assisted secure execution.




allows establishing a trusting relationship with a 

Remote Attestation (RA) is a basic reactive security mechanism for trust establishment and compromise detection in remote entities. 

Remote attestation is a method for software to attest the authenticity of its underlying hardware and the identity of the software to a remote party. Without remote attestation, the trust between SGX enclaves and their users cannot be established.


Remote Attestation (RA) – a distinct security service for detecting malware on CPS, embedded and IoT devices. RA is especially applicable to low-end embedded devices that are incapable of defending themselves against malware infection. This is in contrast to more powerful devices (both embedded and general-purpose) that can avail themselves of sophisticated anti-malware protection. 

RA involves verification of current internal state (i.e., RAM and/or flash) of an untrusted remote hardware platform (prover or P rv) by a trusted entity (verifier or Vrf). If Vrf detects malware presence, Prv’s software can be re-set or rolled back and out-of-band measures can be taken to prevent similar infections. In general, RA can help V rf es- tablish a static or dynamic root of trust in P rv and can also be used to construct other security services, such as software up- dates [43] and secure deletion



The BC emerges as a novel application of distrusted storage, cryptography, communication, and other technologies, which plays a trustworthy role of a decentralized database [38]. All the information is recorded in the form of transactions. All the authorized nodes are able to query or invoke the smart contract to manage the information in the BC database (create, read, update, and delete).
In our protocol, BC maintains a public ledger to record MCs of CRPs for IoT nodes. In addition, Consortium BC [38] employed in our protocol caters to IoT scenarios well, as it is able to reach a consensus with high efficiency and low cost.

Blockchain is a chain that can contain millions of blocks and each block records multiple sets of transaction data in the form of a Merkle tree. Typically, the blockchain is a com- pletely distributed ledger and anyone can gain access to initiate transactions. Once the transactions are logged in a blockchain, it is extremely difficult to alter or remove them. In recent years, blockchain technology has also led to the creation of a series of applications, including smart contracts, decentralized cloud storage, supply-chain communications, and proof of prove- nance. The most famous and practical application is a smart contract, which consists of program codes that take control of the changes in state in the blockchain only if some predefined threshold is achieved. As an example, using a smart contract,
Alice could obtain x cryptocurrency units in a Cryptocurrency Blockchain from Bob with valid computation outcomes.


The first recorded mention of blockchain technology came in a document published in 2008 by the mysterious founder of bit- coin denoted Nakamoto et al. (2008). Basically, blockchain is a time-stamped chain of blocks collectively managed by each par- ticipating node. Every block is cryptographically linked together. Blocks are digitally signed and linked to the previous node, in- cluding their hash value. Blockchain technology has the proper- ties of begin completely distributed, restricted to the given con- tractual code, autonomous and begin traceably. Each node in the blockchain network obtains all the blocks in the chain by con- necting to the neighbor node. Every node in the blockchain has a copy of all nodes. The distributed nature of blockchain allows resistance against any attempt for double-spending or replaying a duplicate transaction. All participate nodes should act according to the rule to reach a consensus. Transaction in the blockchain is im- mutable and cannot be altered once the transaction has been com- pleted and added to the blockchain Fernández-Caramés and Fraga- Lamas (2018).
In addition, blockchain offers a generic, programmable dis- tributed ledger system that tracks the computational outcomes. Zhong et al. (2019). Smart Contract was launched as autonomous systems that are distributed and operate through the blockchain network Rouhani and Deters (2019).


 The important keywords associated with blockchain are the decentraliza- tion, immutability and cryptographic link.

 
Decentralization: The decentralization reflects the trans- actional(store and retrieve data) capability of blockchain based smart contracts without a single point of failure. The ledger is available on each node and in contrast with central- ized database management systems [8], the access to the data does not depend on a centralized service.
Immutability: The records in the ledger are immutable once logged [9]. The attempt to forge the ledger record on a particular block will disqualify it and fail the data integrity of the entire blockchain. The immutability of the ledger ensured using cryptographic techniques such as hashing and digital signatures which will explain in the paper. The alterations of ledger is a computationally expensive task.
Cryptographic Link: The cryptographic link is the back- bone of trust of the entire blockchain [10]. The immutability of blockchain is achieved through the cryptographic link established with hashing and digital signatures [11]. Neither the transaction or block can be altered since it requires alter- ing all subsequent blocks.


Blockchain technology is a decentralized and distributed digital ledger that records transactions across a network of computers in a secure and tamper-proof manner. Each block in the chain contains a cryptographic hash of the previous block, which not only ensures the integrity of the data but also makes it impossible to alter any block in the chain without affecting all subsequent blocks. This feature makes blockchain technology highly secure and resistant to fraud, hacking, and other malicious activities.

Smart contracts, on the other hand, are self-executing digital contracts that are stored on the blockchain. They are created with a set of rules and conditions that automatically execute when the specified conditions are met. Smart contracts are immutable and transparent, meaning that once created, they cannot be modified, and all parties involved can see the terms of the agreement, ensuring a high level of trust and transparency.

However, the adoption of blockchain and smart contracts also presents significant challenges, such as regulatory uncertainty, scalability issues, and the need for widespread adoption. Additionally, while blockchain technology is highly secure, it is not immune to attack, and new vulnerabilities and exploits are constantly being discovered and addressed.

The combination of blockchain and smart contracts has opened up a range of possibilities for various industries, including finance, supply chain management, and real estate. With the ability to create transparent, secure, and efficient systems, blockchain and smart contracts are poised to disrupt traditional business models and bring about a new era of innovation.




The motivation is to improve the scalability of RA in large Pub/Sub IoT networks that  The proposed scheme, called SCRAPS, is a blend of one-to-many and many-to-many approaches that inherit advantages of both. SCRAPS utilizes smart ledger technology to build a decentralized Proxy Verifier – an entity which acts as a proxy and conducts attestation on behalf of actual Verifiers. This allows for better scalability and handles heterogeneous devices while providing on-demand attestation, support for the Pub/Sub networks, sleeping devices, and configuration updates. SCRAPS also accommodates devices with intermittent availability. 

The paper does not explicitly mention any limitations of SCRAPS but acknowledges that their security analysis is informal and future work could include a more rigorous analysis of SCRAPS's security properties. 

Overall, the paper aims to provide a scalable and secure approach to Remote Attestation for IoT devices in a Pub-Sub network with several advantages over existing methods such as better scalability, on-demand attestation, support for heterogeneous platforms and attestation types, and reduced Prover burden.

another hardware based root of trust, 




% The session is no longer for the only two parities but open to every participants.

% pluggable and updated. Then we introduce the audition to enable different parties to sense and even review other sessions.

% "\textbf{publicly executed machine}" "backup audition for historic attestation " 


% 不论是由单个verifier还是一个第三方验证服务给出结果, 声明的能力都始终是一方的, 系统其他参与方很难对历史发生的进行检查或者重新验证

% The basic model of RA where. There have been many efforts on that and the decentralization of original TEE-based RA designs. However, the verificfation results are still claimed by a single party similar to verification service.

% Many studies have been focusing on the basic RA model with only verifiers and attesters. 
% Many This question is two fold: (1) how to let individual verifiers perform evidence validation on their own? (2) how to  claimed by that verifier? For (1), many of RA studies  or the . However, 



This requires .

 A smart contract for different setup targeted cases for different scenarios

 

% Plain RA model: attester may malicious, will fail attestation


% 做个表, 对比, 分类, 用LIRA-V那种G1, G2之类的来搞
%                     protocol attackers             platform attackers
%                     MITM, OS breach, xx, xx, xxx, Attestation Key Compromised, Few Dishonest Verifiers

% traditional model:  

% enhanced model: 

% 1. PUF 
% 2. wrong results
% 3. honest majority

% Advanced model:


% local attestatoin

Here we take two attesters $\att_{\aid_{1}}, \att_{\aid_{2}}$ on the same TEE device as an example to describe this protocol. The two attesters control different enclaves but can both invoke the device's PUF instances.

\noindent\textbf{Sending the local challenge.} We assume that $\att_{\aid_{1}}$ initiates the session and generates the challenge message $(Z_{1}, t_{1})$ by the following step.

\begin{itemize}[itemsep=0pt, parsep=0pt, topsep=2pt]
    \item [\ding{172}] \underline{$(Z_{1}, t_{1})$}:  $\att_{\aid_{1}}$ uses $\aid_{1}$, timestamp $ts_{1}$, local PUF id $\pid_{1}$ and a nonce $n_{1}\in\bin^{n}$ to form $Z_{1}$. Then it uses the PUF instance $\puf{}_{\pid_{1}}$ to get $R_{n_{1}}=\puf{}_{\pid_{1}}(n_{1})$. A standard MAC algorithm $\mathcal{T}$ like HMAC [x] is applied to produce a tag $t_{1}$ on $Z_{1}$ using $R_{n_{1}}$ as the key.
\end{itemize}

\noindent\textbf{Invoking PUF and sending back the measurement.} When receiving $(Z_{1}, t_{1})$ from an untrusted local channel, $\att_{\aid_{2}}$ needs to invoke PUF to verify the tag and respond.

\begin{itemize}[itemsep=0pt, parsep=0pt, topsep=2pt]
    \item [\ding{173}] \underline{verify $(Z_{1}, t_{1})$}:  $\att_{\aid_{2}}$ reproduces the response $R_{n_{1}}$ from $\puf_{\pid_{1}}$ by using $n_{1}$ in the message as the PUF challenge. Therefore, $(Z_{1}, t_{1})$ is considered valid only if they are not modified and the sender can also invoke PUF. The timestamp $ts_{1}$ ensures the freshness of the message. 
    \item [\ding{174}] \underline{$(Z_{2}, t_{2})$}:  After verifying the authenticity of $(Z_{1}, t_{1})$, $\att_{\aid_{2}}$ generates $Z_{2}$ using a different $\pid_{2}$, its enclave measurement $M_{\aid_{2}}$ and other materials. It obtains $R_{n_{2}}=\puf{}_{\pid_{2}}(n_{2})$ and $C_{2}=H(Z_{2}||R_{n_{2}} ||R_{n_{1}})$, then calculates $R_{2}=\puf{}_{\pid_{2}}(C_{2})$ and forms $t_{2}$ eventually. Here the structure of \textit{double hash-double PUF} is similar to HMAC but provides PUF-based integrity and authenticity to the tag generation.
\end{itemize}


\noindent\textbf{Verifying the response and responding mutually.} $\att_{\aid_{1}}$ now needs to respond back as the after verifying the authenticity of $\att_{\aid_{2}}$.

\begin{itemize}[itemsep=0pt, parsep=0pt, topsep=2pt]
    \item [\ding{175}] \underline{verify $(Z_{2}, t_{2})$}:  $\att_{\aid_{1}}$ also uses the specified PUF instance $\puf{}_{\pid_{2}}$ to get $R_{n_{2}}$ and $R_{2}$. Along with the previous $R_{n_{1}}$, it thus verifies the message $(Z_{2}, t_{2})$. Note that we only use the original enclave measurement $M$ here since the generation of $Z_{2}$ already involves PUF. 
    \item [\ding{176}] \underline{$(Z_{3}, t_{3})$}:  $\att_{\aid_{1}}$ follows the same steps in \ding{174} to generate $(Z_{3}, t_{3})$. Its measurement $M_{\aid_{1}}$ is also contained in $Z_{3}$ to attest $\att_{\aid_{2}}$. If the verification passes for both enclaves, it proves that they indeed exist on the same TEE platform.
\end{itemize}

As for step \ding{177}, $\att_{\aid_{2}}$ can verify $(Z_{3}, t_{3})$ as in step \ding{175} and completes the mutual local attestation. $\pid$ can be fixed if only one PUF instance is installed. Our protocol avoids sending PUF responses directly to the channel for attestation, or adversaries can collect enough CRPs to perform ML modeling attacks against PUF. Moreover, $\att_{\aid_{1}}$ and $\att_{\aid_{2}}$ can conveniently use a private PUF response as their shared secret key, eliminating the need of DHKE or other public key operations.




\noindent\textbf{Invoking PUF and sending back the measurement.} 

\noindent\textbf{Verifying the response and responding mutually.} 

As for step \ding{177}, $\att_{\aid_{2}}$ can verify $(Z_{3}, t_{3})$ as in step \ding{175} and completes the mutual local attestation. $\pid$ can be fixed if only one PUF instance is installed. 



A protocol $\pi$ UC-realizes the ideal functionality $\mathcal{F}$, if for any probabilistic polynomial-time (PPT) adversary $\Aa$ there exists a
simulator S such that no PPT environment machine $\mathcal{Z}$ exists to distinguish whether it contacts with $\pi$ and $\Aa$ in the real world or $\mathcal{S}$ and $\mathcal{F}$ in the ideal world. We have,

simulator S such that


emulates the execution of A with an ideal functionality F.

the as the represents for Protocols are represented as interactions between the ideal functionality $\mathcal{F}$ and the Interactive Turing Machines (ITM) that are mathematical abstractions of protocol participants. 
 Its basic idea is to define a computation model where multiple sub-protocols can be composed securely.  Also, a simulator Adversaries are also modeled as ideal functionalities, which capture the worst-case behavior of an attacker.


ideal functionality $\mathcal{F}_{att}$


\begin{figure*}
    \centering
    \begin{mybox}{Functionality: $\mathcal{F}_{att}$}
        \textbf{Initialization}:
        \begin{itemize}[nosep,leftmargin=*]
            \item Upon receiving $(\textsc{Measurement}, \id, \prog)$ from a party $P$, generate platform information $\Ii$ and obtain measurement $m:=\mathsf{memms}(\prog, \Ii)$, then let $\Ll[\id, \prog]:=(\mathsf{measured}, \Ii, m)$ and return $(\textsc{Measured}, \id)$ to $P$.
            % \begin{itemize}[nosep]
            %     \item[-] if receive $(\textsc{Corrupt}, i)$ from $\Ss$, then send $\iid$ to $\Ss$ and set $\Ll[i].\mathsf{state}=\mathsf{invaded}$
            % \end{itemize}
            \item Upon receiving $(\textsc{Provision}, \id)$ from $P$, 
            \begin{enumerate}[nosep, label=(\alph*)]
                \item generate the platform key set $\Kk$ and helper data $\Ww$, update $\Ll[\id, :].\mathsf{append}(\Kk, \Ww)$;
                \item let $\Ll[\id, :].\mathsf{state}=\mathsf{provisioned}$ and return $(\textsc{Provisioned}, \Ww, \id)$ to $P$. 
            \end{enumerate}
            % \begin{itemize}[nosep]
            %     \item[-] if receive $(\textsc{Corrupt}, i)$ from $\Ss$, then send $\kid$ to $\Ss$ and update $\Ll[i, :].\mathsf{state}=\mathsf{compromised}$
            % \end{itemize}
        \end{itemize}
        \textbf{Mutual Attestation}:
        \begin{itemize}[nosep,leftmargin=*]
            \item Upon receiving $(\textsc{Challenge}, i, j, \prog_{i}, \ssid)$ from $P_{i}$,
            \begin{enumerate}[nosep, label=(\alph*)]
                \item send the message to $\Ss$ and update $\Ll[i, \prog_{i}].\mathsf{append}(\ssid)$;
                \item if receive $(\textsc{Challenged}, A, C, T, \ssid)$ from $\Ss$, send it to $P_{j}$ and set $\Ll[j, \prog_{j}].\mathsf{state} = \mathsf{challenged}$.
            \end{enumerate}
            \item Upon receiving $(\textsc{MutAttestation}, i, j, \mathsf{prog}_{j}, \ssid)$ from $P_{j}$,
            \begin{enumerate}[nosep, label=(\alph*)]
                \item send the message along with $(\iid, \prog_{i}, \mathcal{I}_{j}, \prog_{j})$ to $\Ss$ and update $\Ll[j, \prog_{j}].\mathsf{append}(\ssid)$;
                \item if receive $(\textsc{MutAttReport}, \langle A_{i}, C_{i}, T_{i}\rangle, \langle A_{j}, C_{j}, T_{j}\rangle, \sigma_{i}, \sigma_{j}, \ssid)$ from $\Ss$, set $\Ll[i, \prog_{i}].\mathsf{state} = \mathsf{challenged}$. Then send $(\textsc{Attestation}, A_{i}, C_{i}, T_{i}, \mathsf{ssid})$ and $(\textsc{Attestation}, A_{j}, C_{j}, T_{j}, \mathsf{ssid})$ to $P_{i}, P_{j}$, respectively.
            \end{enumerate}
        \end{itemize}
        % let $\sigma\leftarrow \mathsf{PrfGen}(\Kk, \Ii)$ and $C, T\leftarrow\mathsf{Const}(\Kk, \sigma, A)$ accordingly depending on whether $P_{i}$ or $P_{j}$ is honest,. 
        \textbf{Mutual Verification}:
        \begin{itemize}[nosep,leftmargin=*]
            \item Upon receiving $(\textsc{Verification}, i, j, A_{i}, C_{i}, T_{i}, A_{j}, C_{j}, T_{j}, \mathsf{ssid})$ from $P_{i}$ or $P_{j}$, 
            \begin{enumerate}[nosep, label=(\alph*)]
                %\item send the message to $\Ss$;
                \item obtain the signature $\sigma_{i}:=\mathsf{Recov}_{\kid, \wid}(A_{i}, C_{i}, T_{i})$ and $\sigma_{j}:=\mathsf{Recov}_{\Kk_{j}, \Ww_{j}}(A_{j}, C_{j}, T_{j})$; 
                \item if the party is corrputed, or the submitted record and the signature have not appeared or appear more than once, set $f[i, j]:=1$ or $f[j, i]:=1$ accordingly; otherwise let $f[i, j]$ or $f[j, i]$ be the result of $\mathsf{PrfVrf}_{\Kk, \Ww}(\sigma, \Ii, m)$;
                \item set $\Ll[i, \prog_{i}].\mathsf{state}=\Ll[j, \prog_{j}].\mathsf{state}=\mathsf{attested}$ and send $(\textsc{Attested}, f[i, j], \mathsf{ssid})$, $(\textsc{Attested}, f[j, i], \mathsf{ssid})$ to $P_{i}, P_{j}$, respectively.
            \end{enumerate}
        \end{itemize}
        % $\sigma_{i}, \sigma_{j}$ for two parties using $\mathsf{Recov}_{\Kk, \Ww}(A, C, T)$
        % $\sigma_{i}:=\mathsf{Recov}_{\kid, \wid}(A_{i}, C_{i}, T_{i}), \sigma_{j}:=\mathsf{Recov}_{\Kk_{j}, \Ww_{j}}(A_{j}, C_{j}, T_{j})$;
        % \item when receiving $(\textsc{AttReport}, A_{3}, C_{3}, T_{3}, \sigma_{\vid}, \ssid)$ from $\Ss$, if $P_{\vid}$ and $P_{\aid}$ are both honest, let $\sigma_{\vid}\leftarrow \mathsf{PrfGen}(\Kk_{\vid}, \Ii_{\vid})$ and $C_{3}, T_{3}\leftarrow\mathsf{Const}(\Kk_{\vid}, \sigma_{\vid}, A_{3})$.
        % \begin{enumerate}[label=(\alph*), nosep]
        %     \item verify that $\mathsf{aid}, \mathsf{vid}$ has been initialized and $\mathsf{ssid}$ is not shown before. 
        %     \item send $(\textsc{Request}, \mathsf{aid}, \mathsf{vid}, \mathsf{ssid})$ to $\mathcal{S}$.
        % \end{enumerate}
        % check $\id, \id^{'}$ and session id $\ssid$, then
        
    \end{mybox}
    \caption{Ideal Functionality of Mutual Remote Attestation}
    \label{fig:ideal_functionality_Fatt}
\end{figure*}
